Bilingual Problems: Studying the Security Risks Incurred by Native Extensions in Scripting Languages

Scripting languages are continuously gaining popularity due to their ease of use and the flourishing software ecosystems that surround them. These languages offer crash and memory safety by design, thus, developers do not need to understand and prevent low-level security issues like the ones plaguing the C code. However, scripting languages often allow native extensions, which are a way for custom C/C++ code to be invoked directly from the high-level language. While this feature promises several benefits such as increased performance or the reuse of legacy code, it can also break the language's guarantees, e.g., crash-safety. In this work, we first provide a comparative analysis of the security risks of native extension APIs in three popular scripting languages. Additionally, we discuss a novel methodology for studying the misuse of the native extension API. We then perform an in-depth study of npm, an ecosystem which is most exposed to threats introduced by native extensions. We show that vulnerabilities in extensions can be exploited in their embedding library by producing reads of uninitialized memory, hard crashes or memory leaks in 33 npm packages, simply by invoking their API with well-crafted inputs. Moreover, we identify six open-source web applications in which such exploits can be deployed remotely by a weak adversary. Finally, we were assigned seven security advisories for the work presented in this paper, most labeled as high severity.

==> figs/boxplot.tex <==



\begin{figure}
    \centering
\begin{tikzpicture}
\begin{axis} [enlarge x limits=0.2,
xtick=data,
xticklabels={C, H, C++, JS, TS},
xlabel={File types},
ylabel={Number of files per package}, ytick={0,5,10,15,20,25,30,35,40},
ylabel style={yshift=-0.5cm}]
    \addplot [box plot median] table {testdata.dat};
    \addplot [box plot box] table {testdata.dat};
    \addplot [box plot top whisker] table {testdata.dat};
    \addplot [box plot bottom whisker] table {testdata.dat};
\end{axis}
\end{tikzpicture}
    \caption{The number of C/C++ and JavaScript files per package based on file types. 
    C refers to \texttt{.c} files, H indicates header files with \texttt{.h/.hpp} extension, C++ refers to \texttt{.cpp/.cc} files, while JS and TS refer to \texttt{.js} and \texttt{.ts} files, respectively.
    The boxes indicate the lower quartile (25\%) and the upper quartile (75\%) and the whiskers mark the 10\textsuperscript{th} and the 90\textsuperscript{th} percentiles.
    The median should be marked with a horizontal line but it collides with the top (C, H, C++) and/or bottom (C, JS, TS) of the box in all cases.}
    \label{fig:file_types}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}[b]{\columnwidth}
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\draw (0,-0.2) rectangle (10,1.2);
\filldraw[fill=yellow!20] (0,-0.2) rectangle (2.143,1.2);% draw the js box
\filldraw[fill=solaorange!20] (2.143,-0.2) rectangle (10,1.2);% draw the cpp box
\filldraw[fill=solablue!20] (2.143,0.1) rectangle (5,0.9);% draw the box
\node[above] at (2.143,1.2) {\large 21.43\%};
\node[above] at (0,1.2) {\large 0\%};
\node[above] at (10,1.2) {\large 100\%};
\draw (2.143,0.1) -- (2.143,0.9);% draw the median
\draw (0.4301,0.5) -- (2.143,0.5);% draw right whisker
\draw (5,0.5) -- (6.667,0.5);% draw left whisker
\draw (6.667,0.1) -- (6.667,0.9);% draw vertical tab
\draw (0.4301,0.1) -- (0.4301,0.9);% draw vertical tab
%\node[below] at (2,0) {$\textsc{Q1}$};% label the hinge
%\node[below] at (5,0) {$\textsc{Q3}$};% label the hinge
%\filldraw[ball color=red!80,shading=ball] (4,0.5) circle
%(0.06cm) node[above]{$\bar{x}$};% the mean
% Axis
%\draw (-3,-2) -- (11,-2);
% TikZ to draw the final tick.
%\draw[snake=ticks,segment length=1cm] (-3,-2) -- (11.1,-2);
\end{tikzpicture}
}
    \caption{Number of files.}
    \label{fig:percentage1}
\end{subfigure}

\begin{subfigure}[b]{\columnwidth}
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\draw (0,-0.2) rectangle (10,1.2);
\filldraw[fill=yellow!20] (0,-0.2) rectangle (0.591,1.2);% draw the js box
\filldraw[fill=solaorange!20] (0.591,-0.2) rectangle (10,1.2);% draw the cpp box
\filldraw[fill=solablue!20] (0.220,0.1) rectangle (1.943,0.9);% draw the box
\node[above] at (0.9,1.2) {\large 5.91\%};
\node[above] at (0,1.2) {\large 0\%};
\node[above] at (10,1.2) {\large 100\%};
\draw (0.591,0.1) -- (0.591,0.9);% draw the median
\draw (0.035,0.5) -- (0.220,0.5);% draw right whisker
\draw (1.943,0.5) -- (5.011,0.5);% draw left whisker
\draw (5.011,0.1) -- (5.011,0.9);% draw vertical tab
\draw (0.035,0.1) -- (0.035,0.9);% draw vertical tab
\end{tikzpicture}
}
    \caption{Number of lines of code.}
    \label{fig:percentage2}
\end{subfigure}
\caption{The distribution of JavaScript versus C/C++ code in percentage in the studied \nbPkgsStudy{} packages. 
The boxes indicate the lower quartile (25\%) and the upper quartile (75\%) and the whiskers mark the 10\textsuperscript{th} and the 90\textsuperscript{th} percentiles.
The median is marked with a horizontal line and we color the background with yellow (left side of median) for JavaScript and with orange (right side of median) for C/C++ code.}
\label{fig:distribution_perc}
\end{figure}

==> figs/randompackages.tex <==

\begin{figure}
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[
    xbar stacked,
    legend style={
        legend columns=4,
        at={(xticklabel cs:0.5)},
        anchor=north,
        draw=none,
        legend columns=2
    },
    ytick=data,
    axis y line*=none,
    axis x line*=bottom,
    xtick={0,50,100,150,200,250,300},
    width=\columnwidth,
    bar width=5mm,
    xlabel={Time in Seconds},
    yticklabels={Analyst 1,Analyst 2,Analyst 3,Average},
    xmin=0,
    xmax=300,
    area legend,
    y=7mm,
    enlarge y limits={abs=0.625},
]
\addplot[black,fill=red!40] coordinates
% OS
{(191,3) (183,2) (166,1) (180,0)};
\addplot[black,fill=solablue!40] coordinates
% C++
{(74,3) (59,2) (89,1) (74,0)};
\addplot[black,fill=ggreen] coordinates
% Perf
{(27,3) (44,2) (37,1) (36,0)};
\addplot[black,fill=solaorange!40] coordinates
% MISC
{(8,3) (14,2) (8,1) (10,0)};
%\addplot[dashed, sharp plot,update limits=false] coordinates {(104,500) (104,0)};
\legend{Wrap low-level functionality,Wrap C/C++ library,Performance,None}
\end{axis}
%
\draw [dashed,black] (2.35,0) -- (2.35,2.8);
%\draw [thick,red] ({axis cs:1000,0.5} |- {rel axis cs:0,-0.2}) -- ({axis cs:1000,0.5} |- {rel axis cs:0,1.05});
\end{tikzpicture}
}
\caption{Number of packages for each usage category from 300 randomly selected packages. With a dashed line we note the 104 automatically generated packages by NodeRT.}
\label{fig:300categories}
\end{figure}


\begin{comment}
\begin{figure}
    \centering
\begin{tikzpicture}
    \begin{axis}[
        width  = \columnwidth,
        height = 8cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=10pt,
        ymajorgrids = true,
        ylabel = {Run time speed},
        symbolic x coords={Existing C/C++ library,Existing OS/low-level,Performance,None},
        xtick = data,
        x tick label style={rotate=45,anchor=east},
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        legend style={
                at={(1,1.05)},
                anchor=south east,
                column sep=1ex
        }
    ]
        \addplot[style={solablue!40,fill=solablue!40,mark=none}]
            coordinates {
            (Existing C/C++ library, 100) 
            (Existing OS/low-level,150) 
            (Performance,44)
            (None, 6)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {
             (Existing C/C++ library,112) 
             (Existing OS/low-level,156) 
             (Performance,27)
             (None, 5)};

        \addplot[style={solaorange!40,fill=solaorange!40,mark=none}]
             coordinates {
             (Existing C/C++ library,97) 
             (Existing OS/low-level,166) 
             (Performance,29)
             (None, 8)};

                \legend{Analyst 1, Analyst 2, Analyst 3}
    \end{axis}
\end{tikzpicture}
    \caption{Number of packages for each category from 300 randomly selected packages. \agi{Made up numbers for Analyst 1 and 2 now (Sazz and Cris), will fill in later.}}
    \label{fig:my_label}
\end{figure}
\end{comment}


==> figs/venn.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[set/.style={fill=solablue,fill opacity=0.1}]

\draw[set] (0,0) ellipse (2cm and 1cm);

\draw[set, fill=yellow] (2.5,0) ellipse (2cm and 1cm);

\draw[set, fill=solaorange] (0,0) ellipse (3cm and 1.5cm);

\draw[set, fill=green] (2.5,0) ellipse (3cm and 1.5cm);

\draw (2.65,1.25) node {\texttt{node\_api.h}}; 
\draw (-0.5,1.25) node {\texttt{node.h}/\texttt{v8.h}}; 
\draw (3.35,0.6) node {\texttt{napi.h}}; 
\draw (-0.8,0.6) node {\texttt{nan.h}}; 

\draw (1.25,0) node {6}; %intersection of all

\draw (-2.5,0) node {\numprint{1210}}; %node/v8 1210
\draw (-1,0) node {\numprint{4334}}; %nan 1020+3314
\draw (3.75,0) node {526}; %napi 508+18
\draw (5,0) node {179}; %node_api 179

\draw (1.25,1.1) node {7}; %node_api and node/v8
\draw (2.5,0) node {24}; %napi and node/v8
\draw (0,0) node {6}; %nan and node_api

\draw (5,1.3) node {158}; %(none) none + nbind only (18) 

\end{tikzpicture}
\caption{Venn diagram of the identified \nbPkgsStudy{} packages with native extensions, according to if they include \texttt{nan.h} (i.e., use Nan and V8), \texttt{napi.h} (i.e., use node-addon-api and N-API), \texttt{node\_api.h} (i.e., use N-API), or \texttt{node.h}/\texttt{v8.h} (i.e., use~V8). %, not considering redundant includes.
}
\label{fig:venn}
\end{figure}


%%%COMMENTED OUT OLD FIGURE

\begin{comment}
\begin{figure}
\centering
\begin{tikzpicture}[set/.style={fill=solablue,fill opacity=0.1}]
 
% Ellipse 1
\draw[set,
    rotate =45] (0,0) ellipse (2cm and 1cm);

\draw (1,1.8) node {\texttt{node\_api}}; 
\draw (2.5,1.1) node {\texttt{node} or \texttt{v8}}; 
\draw (-1,1.8) node {\texttt{napi}}; 
\draw (-2.5,1.1) node {\texttt{nan}}; 

\draw (0,-0.8) node {0}; %intersection of all

\draw (-0.6,-0.2) node {0}; %intersection of 3 (nodeapi, napi and nan)
\draw (0.6,-0.2) node {2}; %intersection of 3 (nodeapi, napi and nodev8)
\draw (-0.3,-1.25) node {4}; %intersection of 3 (nan, nodeapi and nodev8)
\draw (0.3,-1.25) node {3}; %intersection of 3 (nan, napi and nodev8)

\draw (-1,-1) node {2}; %intersection of 2 (nan and nodeapi) 6-4=2 
\draw (1,-1) node {22}; %intersection of 2 (nodev8 and napi) 27-3-2=22
\draw (0,0.5) node {18}; %intersection of 2 (nodeapi and napi) 20-2=18
\draw (0,-1.8) node {\numprint{3314}}; %intersection of 2 (nodev8 and nan) 3321-4-3=3314
\draw (-1.25,0.45) node {3}; %intersection of 2 (nan and napi) 6-3=3
\draw (1.25,0.45) node {7}; %intersection of 2 (nodev8 and nodeapi) 13-4-2=7

\draw (-1.9,0) node {\numprint{1020}}; %(nan) 4345-4-3-2-3314-3=1019   +1 new
\draw (1.9,0) node {\numprint{1210}}; %(nodev8) 4562-2-3-4-22-3314-7=4552-6-22-3314=1210
\draw (0.9,1.1) node {179}; %(nodeapi) 212-2-4-2-18-7=212-20-13=179
\draw (-0.9,1.1) node {508}; %(napi) 555-2-3-22-18-3=550-40-3=507   +1 new

\draw (2,-1.8) node {158}; %(none) none + nbind only (18)   +2 new

% Ellipse 2
\draw[set, fill=yellow,
    rotate =-45] (0,0) ellipse (2cm and 1cm);
 
% Ellipse 3
\draw[set, fill=green,
    xshift=1cm,
    yshift=-0.705cm,
    rotate =45] (0,0) ellipse (2cm and 1cm);
 
% Ellipse 4
\draw[set, fill=red,
    xshift=-1cm,
    yshift=-0.705cm,
    rotate =-45,] (0,0) ellipse (2cm and 1cm);
 
\end{tikzpicture}
\caption{Venn diagram of the \nbPkgsStudy{} packages that contain C/C++ code, according to if they include \texttt{nan}, \texttt{napi}, \texttt{node\_api}, or \texttt{node}/\texttt{v8}.}
\end{figure}

\end{comment}
